RESQ: A Unified Framework for REliability- and Security Enhancement of Quantized Deep Neural Networks

This work proposes a unified three-stage framework that produces a quantized DNN with balanced fault and attack robustness. The first stage improves attack resilience via fine-tuning that desensitizes feature representations to small input perturbations. The second stage reinforces fault resilience through fault-aware fine-tuning under simulated bit-flip faults. Finally, a lightweight post-training adjustment integrates quantization to enhance efficiency and further mitigate fault sensitivity without degrading attack resilience. Experiments on ResNet18, VGG16, EfficientNet, and Swin-Tiny in CIFAR-10, CIFAR-100, and GTSRB show consistent gains of up to 10.35% in attack resilience and 12.47% in fault resilience, while maintaining competitive accuracy in quantized networks. The results also highlight an asymmetric interaction in which improvements in fault resilience generally increase resilience to adversarial attacks, whereas enhanced adversarial resilience does not necessarily lead to higher fault resilience.

==> draft.tex <==


%%%%%%%%%%%
As the demand for real-time data processing and artificial intelligence (AI) in embedded systems grows, Quantized Deep Neural Networks (QNNs) have emerged as a cornerstone for efficient deployment in resource-constrained environments, ranging from everyday tasks like image classification to mission-critical applications such as autonomous driving \cite{taheri2022dnn, ahmadilivani2023systematic}. 

The ability of QNNs to perform complex computations with reduced precision not only minimizes the computational and memory footprints but also allows for significant energy savings, making them suitable for energy-constrained platforms \cite{taheri2023deepaxe}. 

Despite these advantages, quantization introduces unique challenges related to the accuracy of neural networks. In particular, quantization errors can accumulate, leading to degradation in model performance, especially when deploying models in diverse and unpredictable environments. This is especially critical in applications where accuracy cannot be compromised, such as in autonomous systems or medical diagnostics \cite{yuan2023benchmarking, taheri2024exploration, 10140043}. 

Recent research has made strides in addressing these issues by improving post-training quantization (PTQ) techniques. PTQ is a widely adopted method that compresses QNNs without the need to alter original training procedures or model architectures, thus maintaining the integrity of the initial training process \cite{yuan2023benchmarking}. By reducing the bit-width of weights and activations, PTQ achieves significant memory and computational efficiency. 

To achieve efficient execution of QNN models, a variety of hardware devices such as general-purpose processors (CPUs, GPUs) and specialized accelerators (FPGAs, ASICs) are employed \cite{chen2016eyeriss, jouppi2017datacenter,taheri2024adam1,taheri2024adam0}. 

The extensive memory resources required to store QNN parameters render these systems vulnerable to faults, particularly due to the ongoing miniaturization of transistors \cite{canal2020predictive}. As a result, ensuring the fault tolerance of QNNs deployed on hardware is critical, especially given that even minor errors in parameters can lead to significant drops in accuracy \cite{mittal2020survey, ahmadilivani2023enhancing, ibrahim2020soft, su2023testability}. 

Figure~\ref{intro_RAP-Q} illustrates Fault locations in critical points of a parallel architecture such as the GPUs. Various factors, including temperature fluctuations, radiation, aging of circuits, and electromagnetic interference, can cause these faults. To safely deploy QNNs in such safety-critical systems, enhancing their fault tolerance is essential \cite{ahmadilivani2024systematic, ahmadilivani2023deepvigor, ahmadilivani2024special}. 


Traditional fault-tolerant techniques, like Triple Modular Redundancy (TMR), although effective, introduce significant computational overhead, which can be prohibitive \cite{schorn2018accurate}. Recent research has shifted towards selective hardening approaches, where the focus is on protecting parameters or neurons that have a greater impact on the network’s output \cite{ruospo2021reliability, hanif2020salvagednn, libano2018selective}. 

This selective protection, often determined through resilience analysis, ensures that the most vulnerable components are safeguarded by running them on hardened processing elements. While these methods effectively identify vulnerable components within QNNs, their application has predominantly been limited to FPGA and ASIC platforms, where hardware can be freely modified \cite{abich2022impact, zhao2020ft}. 
\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{picture/GPU.png}
    \caption{Fault locations in critical points of a parallel architecture such as the GPUs \cite{alia2023heavy}}
    \label{intro_RAP-Q}
\end{figure}

However, for many applications, particularly those relying on general-purpose CPUs, GPUs, or fixed accelerator cores, it is often impossible to modify the underlying hardware to enhance the fault tolerance of QNN operations.


An alternative approach to improving QNN fault tolerance involves pruning parameters that correspond to corrupted processing elements, followed by retraining the network \cite{zhang2018analyzing, chitty2020model}. Though this method can be effective, it is specific to the accelerator being used and is not applicable in real-time operations, as it requires pre-diagnosed fault maps generated in a laboratory setting.
\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\textwidth]{picture/methodology-1.png}
    \caption{Proposed methodology for quantizing a DNN model and evaluating its reliability under various fault situations and protections}
    \label{methodology_rap}
\end{figure*}
Other techniques include fault-aware training \cite{cavagnero2022fault, zahid2020fat}, which retrains the entire network with multiple fault injection scenarios, and Error Correction Codes (ECC) \cite{lee2022value} and Algorithm-based Fault Tolerance (ABFT) \cite{zhao2020ft}, which involve data encoding and decoding for real-time fault detection. While these methods can improve resilience, they often introduce significant overhead in terms of memory and computation, limiting their practicality for QNNs.

Activation restriction methods, which limit the propagation of errors through activation functions, have also been proposed \cite{chen2021low, hoang2020ft, ghavami2022fitact}. These methods effectively mitigate error propagation but do not correct errors, leading to failures at high error rates. Additionally, some approaches propose using correction layers that perform redundant computations for error correction, but these can impose a substantial performance burden on QNNs \cite{ali2020erdnn}.

Paper \cite{ahmadilivani2024cost} proposes a model-level hardening approach that inherently integrates error correction into QNN architectures. By selectively duplicating vulnerable channels within convolutional and fully connected layers and introducing an error correction mechanism, the proposed method achieves a level of fault tolerance. However, this method introduces extra memory overhead and requires additional neurons and layers after each protected layer to introduce correction. The other drawback of this model is its software-level manipulation in the original network structure to introduce duplication. 

To address these challenges, this paper presents a comprehensive framework designed to explore the design space of QNNs with a focus on quantization’s impact on reliability, accuracy, memory overhead, and performance. Our framework introduces an innovative fault tolerance technique that utilizes the memory savings from quantization to store critical higher-order bits of parameters within the same memory elements. This approach ensures that the reliability of the QNNs is maintained even in the presence of memory faults, thereby safeguarding against potential accuracy degradation. 



This fault tolerance method is seamlessly integrated into the iterative optimization loop of our framework, enabling the user to define thresholds that balance the trade-offs between reliability and performance. Through extensive experimentation, we demonstrate that QNNs, when subject to post-training quantization without this protection technique, suffer from significant performance degradation, particularly in fault-prone environments. Our results emphasize the critical importance of this technique, which not only provides negative overhead on memory but also optimizes QNN execution on GPUs and other hardware accelerators.

The contributions of this paper are as follows:

\begin{itemize}
    \item \textbf{Design Space Exploration Framework}: We introduce a framework that enables the exploration of the design space to assess the impact of quantization on the reliability, accuracy, memory overhead, and overall performance of QNNs.
    
    \item \textbf{Tailored Negative Overhead Fault Tolerance Technique}: We propose a novel protection technique that leverages the reduced memory from quantization to store critical higher-order bits of parameters within the same memory element, ensuring robustness against faults.
    
    \item \textbf{Optimization for Reliability and Performance}: Our framework provides methods to optimize QNN models based on user-defined design thresholds, enhancing both reliability and performance in real-world applications.
    
    \item \textbf{Empirical Validation}: We empirically demonstrate that QNNs experience significant performance degradation without the proposed protection technique, particularly in fault-prone environments, underscoring the critical nature of our method.
    
    \item \textbf{Memory and Execution Optimization}: We show that the proposed protection technique not only provides a negative overhead on memory but is also optimized for QNN execution.
    
    \item \textbf{Demonstration and Open-Source Framework}: We validate our framework on state-of-the-art deep neural network benchmarks and provide an open-source implementation to facilitate further research and development.
\end{itemize}


The remainder of this paper is structured as follows: Section~II presents the proposed methodology. Section~III discusses the experimental results and the impact of the proposed method on resilience and overhead. Finally, Section~IV concludes the paper.%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
    
As the demand for real-time data processing and artificial intelligence (AI) in embedded systems grows, Quantized Deep Neural Networks (QNNs) have emerged as a cornerstone for efficient deployment in resource-constrained environments, ranging from everyday tasks like image classification to mission-critical applications such as autonomous driving \cite{muhammad2020deep}. The ability of QNNs to perform complex computations with reduced precision not only minimizes the computational and memory footprints but also allows for significant energy savings, making them suitable for energy-constrained platforms \cite{khayami2023impact}.

Despite these advantages, quantization introduces unique challenges related to both the accuracy and reliability of neural networks. In particular, quantization errors can accumulate, leading to degradation in model performance, especially when deploying models in diverse and unpredictable environments. This is especially critical in applications where reliability cannot be compromised, such as in autonomous systems or medical diagnostics \cite{yuan2023benchmarking, khayami2022exploration}. Furthermore, the process of quantization itself is not immune to hardware-induced faults, which can further exacerbate these challenges.

Recent research has made strides in addressing these issues by improving post-training quantization (PTQ) techniques. PTQ is a widely adopted method that compresses QNNs without the need to alter original training procedures or model architectures, thus maintaining the integrity of the initial training process \cite{yuan2023benchmarking}. By reducing the bit-width of weights and activations, PTQ achieves significant memory and computational efficiency. However, the calibration process central to PTQ is highly sensitive to the data distribution, relying on the assumption that the calibration and test datasets share a similar distribution—an assumption often violated in real-world scenarios due to distribution shifts \cite{nagel2020up, khayami2023analytical}.
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{picture/GPU.png}
    \caption{Fault locations in critical points of a parallel architecture such as the GPUs \cite{alia2023heavy}}
    \label{intro_RAP-Q}
\end{figure}
The concept of reliability in QNNs, particularly under varying environmental conditions and in the presence of hardware faults, has become an area of increasing importance. Faults arising from radiation effects, aging, and other environmental stressors can lead to incorrect computations and, in turn, compromise the integrity of the results produced by QNNs \cite{alia2023heavy}. In environments where QNNs are deployed on specialized hardware accelerators like GPUs, the need for robust fault tolerance mechanisms becomes even more pressing \cite{khayami2023impact, khayami2023framework}.

In response to these challenges, this paper presents a comprehensive framework designed to explore the design space of QNNs with a focus on quantization’s impact on reliability, accuracy, memory overhead, and performance. Our framework introduces an innovative fault tolerance technique that utilizes the memory savings from quantization to store critical higher-order bits of parameters within the same memory elements. This approach ensures that the reliability of the QNNs is maintained even in the presence of memory faults, thereby safeguarding against potential accuracy degradation \cite{taheri2022dnn, taheri2023deepaxe, taheri2023appraiser, taheri2023noise}.

This fault tolerance method is seamlessly integrated into the iterative optimization loop of our framework, enabling the user to define thresholds that balance the trade-offs between reliability and performance. Through extensive experimentation, we demonstrate that QNNs, when subject to post-training quantization without this protection technique, suffer from significant performance degradation, particularly in fault-prone environments. Our results emphasize the critical importance of this technique, which not only provides negative overhead on memory but also optimizes QNN execution on GPUs and other hardware accelerators.

The contributions of this paper are as follows:

\begin{itemize}
    \item \textbf{Design Space Exploration Framework}: We introduce a framework that enables the exploration of the design space to assess the impact of quantization on the reliability, accuracy, memory overhead, and overall performance of QNNs.
    
    \item \textbf{Tailored Negative Overhead Fault Tolerance Technique}: We propose a novel protection technique that leverages the reduced memory from quantization to store critical higher-order bits of parameters within the same memory element, ensuring robustness against faults.
    
    \item \textbf{Optimization for Reliability and Performance}: Our framework provides methods to optimize QNN models based on user-defined design thresholds, enhancing both reliability and performance in real-world applications.
    
    \item \textbf{Empirical Validation}: We empirically demonstrate that QNNs experience significant performance degradation without the proposed protection technique, particularly in fault-prone environments, underscoring the critical nature of our method.
    
    \item \textbf{Memory and Execution Optimization}: We show that the proposed protection technique not only provides a negative overhead on memory but is also optimized for QNN execution.
    
    \item \textbf{Demonstration and Open-Source Framework}: We validate our framework on state-of-the-art deep neural network benchmarks and provide an open-source implementation to facilitate further research and development.
\end{itemize}

\section{Related Work}
The reliability of Deep Neural Networks (DNNs) and the impact of quantization have been extensively studied. Various fault models have been explored to understand their effects on different layers and data types within DNNs. For instance, research has shown that reducing data precision, such as using FP16, FP32, and FP64, can enhance GPU performance and efficiency while also improving resilience against faults \cite{basso2020impact}.

Another significant study involved deploying MNIST Convolutional Neural Networks (CNNs) on FPGAs using FP32 and FP16. The findings indicated that lower data precision could substantially improve resilience due to reduced memory usage \cite{libano2021reduced}. Additionally, binary quantization of weights in convolutional layers has been found to decrease vulnerability factors, although it may increase the criticality of faults \cite{libano2020understanding}. Further research highlighted that faults in the most significant bits (MSBs) have a more pronounced impact, especially with aggressive compression \cite{syed2021fault}.

In some cases, the impact of faults in the weight memories of a DNN can be negligible \cite{arechiga2018effect}. However, to gain a deeper understanding of quantization’s impact on DNN reliability, especially in systolic-array-based accelerators, fault injection engines have been developed to simulate faults in activations \cite{taheri2022dnn}.
\end{comment}
\begin{comment}

\section{Introduction}


As the demand for real-time data processing and artificial intelligence (AI) in embedded systems grows, Quantized Deep Neural Networks (QNNs) have emerged as a cornerstone for efficient deployment in resource-constrained environments, ranging from everyday tasks like image classification to mission-critical applications such as autonomous driving \cite{muhammad2020deep}. The ability of QNNs to perform complex computations with reduced precision not only minimizes the computational and memory footprints but also allows for significant energy savings, making them suitable for energy-constraints platforms \cite{khayami2023impact}.

Despite these advantages, quantization introduces unique challenges related to both the accuracy and reliability of neural networks. In particular, quantization errors can accumulate, leading to degradation in model performance, especially when deploying models in diverse and unpredictable environments. This is especially critical in applications where reliability cannot be compromised, such as in autonomous systems or medical diagnostics \cite{yuan2023benchmarking, khayami2022exploration}. Furthermore, the process of quantization itself is not immune to hardware-induced faults, which can further exacerbate these challenges.

Recent research has made strides in addressing these issues by improving post-training quantization (PTQ) techniques. PTQ is a widely adopted method that compresses QNNs without the need to alter original training procedures or model architectures, thus maintaining the integrity of the initial training process \cite{yuan2023benchmarking}. By reducing the bit-width of weights and activations, PTQ achieves significant memory and computational efficiency. However, the calibration process central to PTQ is highly sensitive to the data distribution, relying on the assumption that the calibration and test datasets share a similar distribution—an assumption often violated in real-world scenarios due to distribution shifts \cite{nagel2020up, khayami2023analytical}.
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{picture/GPU.png}
    \caption{Fault locations in critical points of a parallel architecture such as the GPUs \cite{alia2023heavy}}
    \label{intro_RAP-Q}
\end{figure}
The concept of reliability in QNNs, particularly under varying environmental conditions and in the presence of hardware faults, has become an area of increasing importance. Faults arising from radiation effects, aging, and other environmental stressors can lead to incorrect computations and, in turn, compromise the integrity of the results produced by QNNs \cite{alia2023heavy}. In environments where QNNs are deployed on specialized hardware accelerators like GPUs, the need for robust fault tolerance mechanisms becomes even more pressing \cite{khayami2023impact, khayami2023framework}.

In response to these challenges, this paper presents a comprehensive framework designed to explore the design space of QNNs with a focus on quantization's impact on reliability, accuracy, memory overhead, and performance. Our framework introduces an innovative fault tolerance technique that utilizes the memory savings from quantization to store critical higher-order bits of parameters within the same memory elements. This approach ensures that the reliability of the QNNs is maintained even in the presence of memory faults, thereby safeguarding against potential accuracy degradation.

This fault tolerance method is seamlessly integrated into the iterative optimization loop of our framework, enabling the user to define thresholds that balance the trade-offs between reliability and performance. Through extensive experimentation, we demonstrate that QNNs, when subject to post-training quantization without this protection technique, suffer from significant performance degradation, particularly in fault-prone environments. Our results emphasize the critical importance of this technique, which not only provides negative overhead on memory but also optimizes QNN execution on GPUs and other hardware accelerators.

The contributions of this paper are as follows:

\begin{itemize}
    \item \textbf{Design Space Exploration Framework}: We introduce a framework that enables the exploration of the design space to assess the impact of quantization on the reliability, accuracy, memory overhead, and overall performance of QNNs.
    
    \item \textbf{Tailored Negative Overhead Fault Tolerance Technique}: We propose a novel protection technique that leverages the reduced memory from quantization to store critical higher-order bits of parameters within the same memory element, ensuring robustness against faults.
    
    \item \textbf{Optimization for Reliability and Performance}: Our framework provides methods to optimize QNN models based on user-defined design thresholds, enhancing both reliability and performance in real-world applications.
    
    \item \textbf{Empirical Validation}: We empirically demonstrate that QNNs experience significant performance degradation without the proposed protection technique, particularly in fault-prone environments, underscoring the critical nature of our method.
    
    \item \textbf{Memory and Execution Optimization}: We show that the proposed protection technique not only provides a negative overhead on memory but is also optimized for QNN execution.
    
    \item \textbf{Demonstration and Open-Source Framework}: We validate our framework on state-of-the-art deep neural network benchmarks and provide an open-source implementation to facilitate further research and development.
\end{itemize}







\section{Related Work}
\subsection{Quantization}
Quantization is one of the most effective methods to compress neural networks and accelerate their inference \cite{deng2020model}. Quantizing a network means reducing the precision of the weights and activations of the network to make it more computationally efficient while maintaining a similar level of prediction accuracy. The quantized weights and activations are typically stored as integers (such as INT8 and INT4), which reduces the amount of memory required to store them. Lower precision calculations can be performed faster than higher precision calculations, resulting in faster inference times and reduced energy in real-time applications. There are two main types of quantization used for neural networks: Post-Training Quantization (PTQ) and Quantization Aware Training (QAT).

Post-Training Quantization (PTQ) is a quantization technique applied to a pre-trained neural network \cite{banner2019post, choi2018pact, choukroun2019low}. It involves quantizing the weights and activations of the network after training is complete. Quantization Aware Training (QAT) integrates the quantization process into the training process itself \cite{choi2018pact, gong2019differentiable, esser2020learned}. During QAT, the network is trained using a combination of full-precision and lower-precision weights and activations, which helps it learn to be more robust to the effects of quantization. PTQ is generally simpler to implement than QAT, as it involves quantizing a pre-trained network without any additional training. This can be useful in situations where re-training the network with QAT would be time-consuming or impractical \cite{krishnamoorthi2018quantizing}.

Some previous work explores the stability of quantization and the influence of the calibration dataset. \cite{hubara2021accurate} explores the problems of using a small calibration dataset in quantization. PD-Quant \cite{liu2022pd} identifies a disparity between the distribution of calibration activations and their corresponding real activations and proposes a technique for adjusting the calibration activations accordingly. SelectQ \cite{zhang2022selectq} shows that randomly selecting data for calibration in PTQ can result in performance instability and degradation due to activation distribution mismatch. Although prior research explores the impact of the calibration dataset on the performance of quantized neural networks, these investigations focus only on a limited range of factors and their effects on the stability of quantization. This paper presents a framework that enables us to evaluate the reliability of PTQ and conduct a comprehensive analysis of the impact of various factors on the reliability of quantization.

\subsection{Reliability of Neural Networks}
The reliability of deep models becomes an increasingly important topic in recent years, particularly as these models are increasingly used in critical applications such as healthcare, autonomous vehicles, and financial systems. The reliability of deep models is often measured through different dimensions, some commonly used dimensions include: (1) model performance in various situations (including performance on the existing worst categories, noise samples, and out-of-distribution samples, etc.), (2) model robustness against test-time attacks such as adversarial attacks, and (3) the quality of the model's confidence. This paper mainly focuses on the first dimension and leaves the other two as future work. Therefore, here we only give a brief introduction to related works in the first dimension. 

Model reliability in the worst case: Various studies evaluate and improve the reliability of models against worst-case scenarios involving distribution shift and data noise, among other factors \cite{rahimian2019distributionally, han2020survey}. In this context, the evaluation metric typically used is the worst-case accuracy among existing test categories or out-of-distribution (OOD) samples \cite{shen2021towards, han2018co}. It is observed that models trained conventionally with the assumption of independent and identically distributed (IID) data fail to generalize in real-world testing environments with challenges such as hardness, noise, or OOD samples \cite{duchi2018learning, han2018co}. To enhance model reliability in such settings, two common approaches are proposed: (1) explicit employment of robust training paradigms, such as distributionally robust optimization (DRO) and learning with noisy labels (LNL), to enhance model robustness; and (2) implicit data augmentation techniques, such as Mixup \cite{zhang2018mixup}. Despite the efforts made by the community, the model reliability of PTQ methods in such cases remains largely unexplored.
\end{comment}





comments:



mentioning the protecting the only first bit looks suffies, then for the next version we can say why not extenting the number of protection bits

always consider J as one is one idea

statement which mention protecting 5 bits and so on, should get rid of


title:
The paper is about the technique. The framework help exploration ...



The technique allows to find the best quantization considering faul tolerance. 
IF we quantize without the fault tolerance, ... can be part of the discussion


Platform agnoastic or model level fault tolerant technique to emphasize that we are not modifying the platform itself. Hardware accelerator platform agnostic ...

later we can mention that we target GPU

In the exploration of the technique, we can focus on the reliability, accuracy and performance but it should not be in the title. 
